Multi-Dimensional Pruning: Joint Channel, Layer and Block Pruning with Latency Constraint

As we push the boundaries of performance in various vision tasks, the models grow in size correspondingly. To keep up with this growth, we need very aggressive pruning techniques for efficient inference and deployment on edge devices. Existing pruning approaches are limited to channel pruning and struggle with aggressive parameter reductions. In this paper, we propose a novel multi-dimensional pruning framework that jointly optimizes pruning across channels, layers, and blocks while adhering to latency constraints. We develop a latency modeling technique that accurately captures model-wide latency variations during pruning, which is crucial for achieving an optimal latency-accuracy trade-offs at high pruning ratio. We reformulate pruning as a Mixed-Integer Nonlinear Program (MINLP) to efficiently determine the optimal pruned structure with only a single pass. Our extensive results demonstrate substantial improvements over previous methods, particularly at large pruning ratios. In classification, our method significantly outperforms prior art HALP with a Top-1 accuracy of 70.0(v.s. 68.6) and an FPS of 5262 im/s(v.s. 4101 im/s). In 3D object detection, we establish a new state-of-the-art by pruning StreamPETR at a 45% pruning ratio, achieving higher FPS (37.3 vs. 31.7) and mAP (0.451 vs. 0.449) than the dense baseline.

==> sec/1_intro_bullet.tex <==
\section{Introduction}
\begin{itemize}
    \item \textbf{Background.} CNNs have shown great progress in vision tasks. Though Transformers getting popular, CNNs are still heavily relied on. 
    \item \textbf{Motivations.} Models getting bigger, which easily exceed the capability of edge computing devices. Challenging for realtime task like Autonomous driving and very costly in cloud computing. Pruning is useful by removing parameters. To deploy large models on edge devices, we need an aggressive parameter reduction. 
    \item  \textbf{Current Method and Limitations.} Channel pruning has been explored as an effective approach to accelerate CNNs. However, two issues:
    \begin{itemize}
        \item Approaches usually tackle moderate pruning ratios. Fall short with larger pruning since they can not handle block or layer removal. Refer to some related papers here. They are only confined to prune at layer or block granularity or require training additional parameters from scratch. 
        \item FLOPs and parameter counts not directly related to model latency. For recent hardware pruning methods (HALP, SMCP), latency is inaccurately estimated. (Concretely, this is because they only focus on the latency impacts from reducing output channels of a layer, neglecting the fact that the input channel count could be simultaneously changing.) This inaccuracy leads to suboptimal accuracy v.s. latency. This weakness also gets more severe in large pruning where accurate latency modeling is needed to precisely guide pruning procedure. 
        
    \end{itemize}
    To mitigate the above two issues, methods are carried out in an iterative manner, introducing complexity to the process.
    \item \textbf{Our Method.} We propose a method which solves the above issues:
    \begin{itemize}
        \item We go beyond mere channel pruning and incorporate layer and block as “group” to simultaneously determine optimal sparse architectures on both channel and block levels.
        \item We design methods to more accurately estimate latency reduction from pruning. Concretely, simultaneously capturing variations in both input and output channels.
    \end{itemize}
    Combine the above two into a joint optimization described by a MINLP, which can be solved with only a single pass.

    \item \textbf{Experiments.} We conduct extensive experiments. We show our methods beat the baseline current methods by a margin, \textit{especially at large pruning ratios with high latency.}
    \begin{itemize}
        \item In ablation, we first ablate on the above two fixes (block pruning and more accurate latency estimation) to understand each individual effect. We also show how oneshot and iterative affect our algorithm performance.
    \end{itemize}
\end{itemize}


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/HALPv2-framework.pdf}
    \caption{Paradigm of our proposed method.}
    \label{fig:paradigm}
\end{figure}


\begin{figure}[t!]
\begin{subfigure}[b]{.5\textwidth}
\begin{center}
   \includegraphics[width=\linewidth]{figs/teaser.pdf}
\end{center}
\end{subfigure}
\hfill
\begin{subfigure}[b]{.47\textwidth}
\begin{center}
   \includegraphics[width=\linewidth]{figs/streampetr (1).pdf}
\end{center}
\end{subfigure}
\caption{Pruning results on ImageNet with ResNet50(left) and on NuScenes with StreamPETR(right). Our method consistently achieves better accuracy-latency tradeoffs than the previous methods, especially at large pruning ratios with high latency. Top-right is better.}
\label{fig:teaser}
\vspace{-10pt}
\end{figure}



==> sec/2_related_bullet.tex <==
% A plethora of pruning methods has yielded profound progresses in model compression~\cite{lecun1990optimal, han2015deep, gale2019state, zhou2021effective, sun2022disparse}, providing practical speedup and memory benefits~\cite{li2017pruning, molchanov2019importance, he2020learning, lin2020hrank} through hardware-friendly sparsity~\cite{wu2020constraint, li2020eagleeye, shen2021halp, humble2022soft, shen2023hardware} that trades off accuracy and performance  via FLOPs/latency. Our work can be categorized into the field of model pruning. In this section, we will provide a recap of pruning and discuss the latest methods in the field.
\section{Related Works}
\label{sec:related}
Our work can be categorized as a pruning method. 
\textbf{Channel Pruning}
  \begin{enumerate}
      \item A brief overview of the field. Then introduce channel pruning.
  \end{enumerate}
  
\noindent\textbf{Layer and Block Pruning}
\begin{enumerate}
    \item Explain that channel pruning is only limited to channel level and a moderate pruning ratio. At large pruning ratio, we need to remove block and layer.
    \item Not a lot of works focusing on this. Cite the few works in this direction. 
    \item Mention alternative ways to achieve this. Some automl and NAS approaches. Rely on a very computationally expensive searching and enumeration process.
    \item Discuss our difference. We do not need any training from scratch and tackle from an optimization perspective. We consider layer and block as "group" in optimization.
\end{enumerate}


\noindent\textbf{Hardware-aware Pruning} Since both parameter counts or FLOPs do not directly translate into latency, latest methods go one step further and perform hardware-aware pruning which aims to directly reduce the hardware inference latency. 
\begin{enumerate}
    \item Mention and describe the HALP, SMCP, and the IV paper. Discuss how they set up the Knapsack problem to solve the pruning objective.
    \item Discuss their limitations. Latency estimation is inaccurate. Describe that only latency impact from reducing output channels is considered, but neglecting simultaneous variations in both input and output. (Concretely, when we prune output channels for a layer, the input channel count for its connected subsequent layer also changes, but this is not captured. Mention we show detailed formulation in Appendix to explain this.)
    \item Discuss our differences. We introduce layer latency matrix to simultaneously capture the impacts on latency from both input and output channel levels and globally solve the optimal channel counts for all layers with joint optimization.
\end{enumerate}

\noindent\textbf{Mixed-Integer Nonlinear Program (MINLP)~\cite{lee2011mixed, burer2012non, bussieck2003mixed}} Since the backbone of our proposed formulation is a MINLP, we will now briefly introduce the field. 
\begin{enumerate}
    \item Explain the definition of MINLP
    \item What are the common solvers for MINLP?
    \item Which solver do we use?
\end{enumerate}
  
  % Though achieving decent accuracy and speedups on various datasets, these methods~\cite{shen2021halp, shen2023hardware, humble2022soft} start to exhibit severe performance drops with large latency reduction ratio or one-shot pruning, which are limited by two main criteria. First, their optimization framework itself is inaccurate and does not include all variables affecting parameter latency. For example, inference latency of a convolution layer can be characterized by two prunable parameters: number of input channels and output channels, whereas they~\cite{shen2021halp, humble2022soft, shen2023hardware} only include the number of output channels into their mathematical modeling. Second, they are incapable of handling hierarchical changes in pruning, like the removal of an entire residual block. Notably, we find that this hierarchical unawareness is also a common issue in almost all other pruning methods~\cite{molchanov2019importance, he2019filter, lin2020hrank, wimmer2022interspace, li2023differentiable}. Our work also focuses on the hardware-aware pruning setting and presents a novel pruning framework that effectively addresses the above issues.


==> sec/3_method_bullet.tex <==
\section{Methodology}
\noindent\textbf{Notations}
\begin{enumerate}
    \item Define some terms and expressions
    \item Use a table to declare notations. More organized and clear.
    \item Explain each notation briefly.
\end{enumerate}

\subsection{Method Name}
State our problem. Go over the method. Our method consists of four steps. Given a pretrained model and a desired latency budget, we simply carry out the following four steps.

Here we will describe each of the four stages in our algorithm. 

\noindent\textbf{Step 1: Compute Configuration Importance.}
\begin{enumerate}
    \item Discuss how we measure channel importance score
    \item Discuss how we go from channel importance score to layer configuration importance
\end{enumerate}
\noindent\textbf{Step 2: Construct Latency Matrices.}
\begin{enumerate}
    \item Discuss how we construct the latency matrix for each layer from a lookup table
    \item \textit{This is one of our important features.} Discuss how this captures variations in both input and output channels, and a bit comparison with HALP.
\end{enumerate}

\noindent\textbf{Step 3: Group Block}
\begin{enumerate}
    \item Discuss how we group channels belonging to the same block together.
    \item \textit{This is one of our important features.} Discuss what this grouping will do in optimization, and what benefits come from this?
\end{enumerate}

\noindent\textbf{Step 4: Solve MINLP}
\begin{enumerate}
    \item Present the optimization problem we solve
    \item Discuss how to input it into the MINLP solver
    \item Discuss a few constraints we need to consider.
\end{enumerate}

Present the pseudo code.
% Although we prevent layers from getting completely pruned, the block decision variables with higher priority will remove the entire 

==> sec/4_exp_bullet.tex <==
\section{Experiments}

To validate our proposed method, we perform extensive experiments across a comprehensive set of scenarios. 
\begin{enumerate}
    \item  Results on the image classification task with ImageNet~\cite{deng2009imagenet} and ResNet50~\cite{he2016deep}
    \item 2D object detection task with Pascal VOC~\cite{everingham2010pascal}
    \item 3D object detection task with Nuscenes~\cite{caesar2020nuscenes} and StreamPETR~\cite{wang2023exploring}
    \item Discuss baselines we compare. Under what settings
    \item Also conducted an in-depth ablation study, highlighting the contributions of our block grouping and more accurate latency pruning individually.
\end{enumerate}

Go over the optimization and experiment settings. On what device, PyTorch, GPU...

\textbf{Results on ImageNet}
\begin{enumerate}
    \item Table~\ref{table:imageresnet50}
    \item Describe evaluation metrics
    \item Discuss the results. Particularly compared with HALP and SMCP.
    \item Particularly excels when targeting high FPS at aggressive pruning ratio, validating the effectiveness.
\end{enumerate}

\begin{table*}[ht!]
    \centering
    \vspace{-0.2cm}
    % \resizebox{.85\textwidth}{!}
    {
        % \begin{tabular}{c|cccc}
        \begin{tabular}{lcccc}
            \toprule
            \rowcolor{lgray} 
            \textsc{Method} & \textsc{Top-1 Acc}($\%$)$\uparrow$ & \textsc{Top-5 Acc}($\%$)$\uparrow$  & \textsc{FLOPs}($\times e^9$)$\downarrow$ & \textsc{FPS(im/s)}$\uparrow$ \\
            % {\footnotesize (baseline)}
            \midrule
            \multicolumn{5}{c}{\textbf{ResNet50~\cite{he2016deep}}}\\
            \textsc{Dense} & $76.2$&$92.9$ & $4.1$&$1019$\\
            \midrule
            \textsc{MetaPrune}\cite{liu2019metapruning} & $73.4$ & --& $1.0$ & $2381$ \\
            \textsc{AutoSlim}\cite{yu2019autoslim} & $74.0$ & --& $1.0$ & $2390$ \\
            \textsc{GReg-2}\cite{wang2021neural} & $73.9$ & --& $1.3$ & $1514$ \\
            \textsc{HALP-$30\%$}\cite{shen2021halp} & $74.5$ &$91.8$ & $1.2$ & $2597$ \\
            \textsc{SMCP-$30\%$}\cite{humble2022soft} & $\mathbf{74.6}$ &$92.0$ & $1.0$ & $2947$ \\
            %\textsc{HALP*-$30\%$} & $74.5$ &$92.0$& $1.1$ & $2488$ & $90+90$&\cmark\\
            \rowcolor{lgreen} \textbf{\textsc{Ours-30\%}} & $\mathbf{74.6}$ &$\mathbf{92.2}$ & $1.1$ & $\mathbf{3092}$ \\
            \midrule
            \textsc{HALP-$15\%$}\cite{shen2021halp} & $68.1$ &$88.4$& $0.6$ & $3971$ \\
            \rowcolor{lgreen} \textbf{\textsc{Ours-15\%}} & $\mathbf{70.0}$ &$\mathbf{89.3}$& $0.5$ & $\mathbf{5306}$ \\
            \midrule
            \midrule
            \multicolumn{5}{c}{\textbf{ResNet50 - EagleEye~\cite{li2020eagleeye}}}\\
            \textsc{Dense}~\cite{li2020eagleeye} & $77.2$ &$93.7$& $4.1$&$1019$\\
            \bottomrule
 \textsc{EagleEye-1G}\cite{li2020eagleeye} & $74.2$ &$91.8$ & $1.0$ & $2429$ \\
 \textsc{HALP-30\%}\cite{shen2021halp} & $74.5$ &$91.9$ & $1.2$ & $2597$ \\
  \textsc{SMCP-30\%}\cite{humble2022soft} & $75.1$ &$92.3$ & $1.1$ & $2589$ \\
    \rowcolor{lgreen}
  \textbf{\textsc{Ours-35\%}} & $\mathbf{75.2}$ &$\mathbf{92.5}$& $1.3$ & $\mathbf{2774}$ \\
  \rowcolor{lgreen}
  \textbf{\textsc{Ours-30\%}} & $75.0$ &$92.2$& $1.2$ & $3052$ \\
  \midrule
  % \textsc{SMCP-25\%}\cite{humble2022soft} & $74.4$ &$92.0$ & $0.9$ & $3102$ \\
  \textsc{HALP-20\%}\cite{shen2021halp} & $71.2$ &$90.1$& $0.7$ & $3691$ \\
  \textsc{SMCP-20\%}\cite{humble2022soft} & $72.7$ &--& --& $3784$ \\
  \rowcolor{lgreen}
  \textbf{\textsc{Ours-20\%}} & $\mathbf{72.8}$ &$\mathbf{90.9}$& $0.7$ & $\mathbf{4210}$ \\
  \midrule
\textsc{HALP-15\%}\cite{shen2021halp} & $68.6$ &$88.5$& $0.6$ & $4101$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-15\%}} & $\mathbf{70.0}$ &$\mathbf{89.2}$& $0.5$ & $\mathbf{5262}$ \\
\bottomrule
        \end{tabular}
    }
    \caption{\textbf{ImageNet results with ResNet-50}. FPS is measured on NVIDIA TITAN V. Results with similar FPS are grouped. Ours achieve much better accuracy-FPS tradeoffs than the baselines, specifically when pruning ratio is large. Averaged results over two runs.}
    \label{table:imageresnet50}
\end{table*}

\begin{figure}[ht!]
\begin{center}
   \includegraphics[width=.5\linewidth]{figs/pascalvoc.pdf}
\end{center}
\vspace{-5pt}
\caption{\textbf{PascalVOC results with SSD512}. Results of FPS versus mAP are plotted (left, top-right is better). FPS is measured on NVIDIA TITAN V. Ours achieve much better accuracy-FPS tradeoffs than the baselines.}
\label{fig:pascal}
\end{figure}
\textbf{Results on PascalVOC} 
\begin{enumerate}
    \item Figure~\ref{fig:pascal}
    \item Describe evaluation metrics
    \item Describe the Pareto Frontier is much better. Discuss the results and compare with SMCP.
\end{enumerate}

\begin{table*}[ht!]
\centering
\begin{tabular}{c|c|c|ccccc|c}
\toprule
\rowcolor{lgray}
\textsc{Method} & \textsc{mAP$\uparrow$} & \textsc{NDS$\uparrow$} & \textsc{mATE$\downarrow$} & \textsc{mASE$\downarrow$} & \textsc{mAOE$\downarrow$} & \textsc{mAVE$\downarrow$} & \textsc{mAAE$\downarrow$} & \textsc{FPS$\uparrow$} \\
\midrule
\textsc{BEVPoolv2}\cite{huang2022bevpoolv2} & $0.406$ & $0.526$ & $0.572$ & $0.275$ & $0.463$ & $0.275$ & $0.188$ & $16.6$ \\
\textsc{BEVDet4D}\cite{huang2022bevdet4d}& $0.322$ & $0.457$ & $0.703$ & $0.278$ & $0.495$ & $0.354$ & $0.206$ & $16.7$ \\
\textsc{PETRv2}\cite{liu2023petrv2} & $0.349$ & $0.456$ & $0.700$ & $0.275$ & $0.580$ & $0.437$ & $0.187$ & $18.9$ \\
\textsc{Sparse4Dv2}\cite{lin2023sparse4d} & $0.439$ & $0.539$ & $0.598$ & $0.270$ & $0.475$ & $0.282$ & $0.179$ & $20.3$ \\
\textsc{StreamPETR}\cite{wang2023exploring} & $0.449$ & $0.546$ & $0.613$ & $0.267$ & $0.413$ & $0.265$ & $0.196$ & $31.7$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-55\%}} & $\mathbf{0.451}$ & $\mathbf{0.551}$ & 0.596& 0.272& 0.413& $0.259$& $0.207$& $\mathbf{37.3}$ \\
\midrule
\textsc{HALP-50\%}~\cite{shen2021halp} & $0.439$ & $0.543$ & 0.605 & 0.270 & 0.419 & 0.265 & 0.211 & $38.6$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-50\%}} & $\mathbf{0.441}$ & $\mathbf{0.544}$ & 0.606 & 0.269 & 0.421 & 0.268 & 0.205& $\mathbf{39.0}$ \\
\midrule
\textsc{HALP-40\%}~\cite{shen2021halp} & $\mathbf{0.427}$ & $\mathbf{0.533}$ & 0.620 & 0.269 & 0.438 & 0.271 &0.209 &$39.5$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-40\%}} & $\mathbf{0.427}$ & $0.532$ & 0.608 &  0.272 & 0.457 &0.269 &0.207 & $\mathbf{40.7}$ \\
\midrule
\textsc{HALP-30\%}~\cite{shen2021halp} & $0.373$ & $0.489$ & 0.674 & 0.277 & 0.534 & 0.293 & 0.197 & $42.5$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-30\%}} & $\mathbf{0.394}$ & $\mathbf{0.512}$ & 0.642 & 0.275 & 0.449 & 0.278 & 0.204 & $\mathbf{43.3}$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Nuscenes results with StreamPETR}. FPS is measured on NVIDIA GeForce RTX 3090. Results with similar FPS are grouped. Ours achieve much better accuracy-FPS tradeoffs than HALP and even surpass performance of dense StreamPETR with much higher FPS.}
\label{table:nuscenes}
\end{table*}
\textbf{Results on Nuscenes}
\begin{enumerate}
    \item Motivate again why we show this result. This is on the very latest modern 3D detection model with transformers. Our algorithm could enhance the accuracy-latency even for this hybrid structure. Report FPS of CNNs v.s. Transformers from SteamPETR.
    \item Table ~\ref{table:nuscenes}
    \item Describe evaluation metrics
    \item Discuss the results. Compared with HALP, the advantage is more obvious at large pruning, again validating our effectiveness.
    \item Even improve baseline StreamPETR result with the $-55\%$ settings.
\end{enumerate}

\subsection{Ablation Study}
Explain how we conduct ablation. Compared with pruning methods like HALP, our features are:
\begin{enumerate}
    \item Block Grouping
    \item Layer Latency Matrices
\end{enumerate}
We ablate each of them to study individual effects.


\noindent\textbf{Block Grouping}
\begin{enumerate}
    \item Figure \ref{fig:ablation}
    \item Discuss how this setting is run. Relate to the Methodology section.
    \item Discuss the results. Block grouping individually brings benefits.
    \item \alex{Maybe we also add another plot showing the pruned structure distribution here. Or this can be included in the Appendix?}
\end{enumerate}

\noindent\textbf{Layer Latency Matrices}
\begin{enumerate}
    \item Figure \ref{fig:ablation}
    \item Discuss how this setting is run. Relate to the Methodology section.
    \item Discuss the results. Using layer latency matrices individually brings benefits.
\end{enumerate}

\noindent\textbf{One-shot versus Iterative Pruning} 
\begin{enumerate}
    \item Discuss if we use iterative pruning for our setting instead what will be the difference.
    \item \alex{Figure \ref{fig:ablation} missing one line}
    \item Table \ref{table:ablation} goes into a bit more detail and study how different steps affect the performance. HALP collapses with one shot.
\end{enumerate}


\begin{table}[t!]
\centering
\begin{tabular}{c|clcc}
\toprule
\rowcolor{lgray}
\textsc{Method} & \textsc{Steps} &\textsc{Ratio}& \textsc{Top-1$\uparrow$}& \textsc{FPS$\uparrow$} \\
\midrule
\textsc{HALP}\cite{shen2021halp} & $30$  &70& $74.3$ & $2505$ \\
\textsc{HALP}\cite{shen2021halp} & $10$  &70& $73.9$ & $2622$ \\
\textsc{HALP}\cite{shen2021halp} & $1$  &70& $65.1$ & $4444$ \\
\hdashline
\textbf{\textsc{Ours}} & $30$  &70& $74.5$ & $2660$ \\
\textbf{\textsc{Ours}} & $10$  &70& $74.8$ & $2860$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours}} & $1$  &70& $75.2$ & $2774$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation study results on ImageNet with ResNet50}. Results of HALP~\cite{shen2021halp} and ours with different pruning steps are shown with a pruning ratio of $70\%$. One-shot pruning correspond to Steps of 1. HALP is completely not functioning with one-shot or smaller pruning steps.}
\label{table:ablation}
\end{table}

\begin{figure}[t!]
\begin{center}
   \includegraphics[width=.5\linewidth]{figs/Ablation3.pdf}
\end{center}
\vspace{-5pt}
\caption{\textbf{Abaltion study results on ImageNet with ResNet50}. We ablate on our method and show the results of each component of our formulation operating independently. Top-right is better.}
\label{fig:ablation}
\end{figure}

==> sec_cached/1_intro.tex <==
\section{Introduction}
% \textbf{Task and Motivations} 

% Models keep growing, and we need a large pruning ratio to bring them to edge devices. This is influential since (1) it enables real-time inference on edge computing useful to cases like auto-driving (2) yields dollar savings on cloud computing. 

% Effectively pruning convolution layers is still impactful. Modern networks like StreamPETR use transformers as decoders and a heavy CNN component for feature extraction. (ToDO: Include inference time of the two parts for StreamPETR model.)
Convolutional Neural Networks (CNNs) have become the de-facto standards of advanced computer vision applications, ranging from image classification~\cite{he2016deep} to object detection~\cite{liu2016ssd} and segmentation~\cite{long2015fully}. As the field advances, pushing the boundaries of performance, the models swell in size correspondingly, containing millions or even billions of parameters~\cite{kirillov2023segment}. To ensure these expansive models are deployable on edge devices, which are bound by limited computational resources, a \emph{more aggressive parameter reduction} is crucial to meet the target resource constraints. This is particularly vital in applications such as autonomous driving~\cite{shen2023hardware}, where realtime inference is not merely an advantage but a safety imperative. Even on the cloud computing platforms, pruning a significant number of parameters not only expedites processing but also leads to significant dollar savings for users due to the increased model throughput.

While Transformers~\cite{dosovitskiy2020image} are trendy, contemporary networks continue to depend on convolution layers for feature extraction. For example, StreamPeTR~\cite{wang2023exploring}, the latest state of the art in 3D object detection, utilizes transformers as decoders yet relies on a heavy CNN component for feature extraction. Consequently, substantially pruning CNNs is still crucial for boosting the efficiency of modern systems.

% \textbf{Methods and limitations}

% First one or two sentences to introduce pruning. Although they show promising results, they focus on low prune ratios. They fail to maintain performance at the large pruning ratio. Current methods only consider pruning at channel levels. When it comes to large pruning, we can not avoid removing blocks/layers to achieve competitive results. Here, we include a figure to illustrate block/layer removal. This is the issue (i).

% To enable this, we require some careful considerations. If we do not impose any structural constraint to the pruning process, removing an entire layer like Conv. Layer 2 could “disconnect” the model leading to “NaN” in training loss.
% Second. Parameters and latency are not correlated. There has been a large number of methods aiming at optimizing latency directly, and they rely on extracting latency cost from a pre-built LUT which records inference latency for a convolution layer with certain number of input/output channels. However, prior methods make poor use of the LUT. Make an example here that HALP only considers impact of output channels to the latency. This leads to inaccurate latency estimation for pruned architecture, which yields sub-optimal pruning results. This is the issue (ii).
% Due to (i) and (ii), both methods need to be carried out iteratively to somewhat mitigate the weaknesses as much as possible, which requires extra hyperparameter tuning effort and complicates the process. (We could also mention that this requires solving optimization problems multiple times thus add some overhead as well.)

Channel pruning~\cite{li2017pruning,shen2021halp,humble2022soft,molchanov2019importance, li2020eagleeye, wang2021neural, shen2021when, shen2023hardware}, in particular, has garnered significant attention as an effective technique to practically reduce model complexity without significantly compromising its accuracy. It involves removing redundant convolution channels identified by some importance criterion~\cite{molchanov2019importance, li2017pruning, lin2020hrank} from a pre-trained model and subsequently fine-tuning it. 
\begin{figure}[t!]
\begin{center}
   \includegraphics[width=\linewidth]{figs/teaser.pdf}
\end{center}
\vspace{-5pt}
\caption{Pruning results on ImageNet with ResNet50. Our method consistently achieves better accuracy-latency tradeoffs than the previous methods, especially at large pruning ratios with high latency. Top-right is better.}
\label{fig:teaser}
\vspace{-10pt}
\end{figure}
Despite advancements, existing methods typically target moderate pruning ratios (30\%-50\%) and fall short when tasked with more aggressive reductions of parameters (70\%-90\%). These methods are confined to pruning on the channel level, while we can not avoid structural removal of entire blocks or layers at larger pruning ratios to achieve competitive results with the desired computation reduction. However, there are a very limited number of methodologies~\cite{xu2020layer, yu2022unified} that address pruning on layer or block levels, and all of them add extra shortcut connections and parameters to the model, with the expectation of training these additions from scratch. This is infeasible when only a pre-trained model is available. \textit{\textbf{(i)}} \emph{Therefore, achieving high-performance models at a large pruning ratio is still a challenge.}

Furthermore, most existing pruning methods~\cite{li2017pruning,molchanov2019importance, wang2021neural, lin2020hrank, fang2023depgraph} aim to remove as many parameters as possible from neural network models or use computational proxies like Floating Point Operations (FLOPs)~\cite{li2020eagleeye, wu2020constraint,yu2019autoslim} to improve pruning effectiveness. However, recent studies~\cite{tan2019mnasnet, shen2021halp} have revealed that neither parameter counts nor FLOPs directly correlate with hardware latency, creating challenges in achieving actual practical speedups through pruning. Therefore, newer approaches~\cite{shen2021halp,humble2022soft,castro2022probing,chen2022lap,kong2022spvit,yang2023global,molchanov2022lana,shen2023hardware} are shifting towards hardware-aware pruning, which targets directly reducing the actual inference latency on hardware. These methods~\cite{shen2021halp, humble2022soft, shen2023hardware} use a pre-built latency lookup table to evaluate the latency cost of each convolution channel, formulating pruning as a knapsack problem~\cite{sinha1979multiple}, maximizing total channel importance under latency constraint.

Nevertheless, these approaches have their shortcomings. They primarily focus on the impact of reducing output channels on layer's latency, neglecting the simultaneous changes in both input and output channels of convolution layers during pruning. \textit{\textbf{(ii) }This oversight can lead to pruned models not performing as quickly on hardware as anticipated, resulting in suboptimal trade-offs between accuracy and latency.}

To somewhat mitigate these limitations \textbf{(i) and (ii)}, pruning techniques are often carried out in an iterative manner~\cite{han2015deep, molchanov2019importance, shen2021halp}, gradually achieving the target compression ratio with some designed scheduler~\cite{de2020progressive} involving multiple rounds of pruning and finetuning sessions. Though usually yielding better performance than one-shot pruning, it introduces additional hyperparameters and necessitates more tuning efforts, which adds complexity to the pruning process.

% \textbf{Your idea/Solution}
% We propose a novel pruning framework to simultaneously address both issues (i) and (ii). 
% To properly consider structural change like removing a block all at once, we directly formulate it into our pruner. This allows us to directly solve for a globally optimal pruned structure in both channels and block space. 
% To precisely capture the latency cost associated with a particular pruned structure, we transform the LUT to capture the variations of latency with both input and output channels changing.
% To enable these, we re-formulate the pruning process as a Mixed-Integer Nonlinear Program (MINLP), which simply needs to be solved once to determine a globally optimal pruned structure from the pre-trained weights. , which can be efficiently solved by numeric solver~\cite{bynum2021pyomo, bernal2018mixed} within seconds
In this paper, we present an innovative and highly effective pruning framework that simultaneously addresses both prior major limitations \textbf{(i) and (ii)}. We revisit the pruning formulation and incorporate blocks as groups to determine an optimal pruned structure on both channel and block space. To precisely capture the latency cost of each layer to guide pruning, we construct a \emph{layer latency matrix} for each layer which describes its variations in inference latency with different input and output channel counts. We organically integrate the above solutions into our pruning strategy by re-formulating pruning as a Mixed-Integer Nonlinear Program (MINLP)~\cite{lee2011mixed, burer2012non, bussieck2003mixed} to directly achieve the optimal pruned structure adhering to a specific latency budget. Notably, our method can prune the model with \emph{only a single shot}, streamlining the process significantly.

% \textbf{Proof it works}
% Briefly introduce our experiments. Tease with a good result. Refer to the teaser Figure 1. Introduce our ablation experiment. Combining fixes for both (i) and (ii) yields the best result.
To validate the efficacy of our proposed method, we conduct extensive experiments and observe state-of-the-art accuracy-latency trade-offs in a wide range of settings, covering (a) ImageNet~\cite{deng2009imagenet} for classification, Pascal VOC~\cite{everingham2010pascal} for 2D detection, and Nuscenes~\cite{caesar2020nuscenes} for 3D detection (b) with three model architectures: ResNet-50~\cite{he2016deep}, SSD~\cite{liu2016ssd}, and StreamPETR~\cite{wang2023exploring} (c) across various latency reduction pruning ratios. We provide a glimpse of our comprehensive results in Figure~\ref{fig:teaser} which clearly indicates that our method exceeds existing techniques by a large margin, especially at \emph{large pruning ratios with high latency}. 

We summarize our key contributions as follows:
\begin{itemize}
    \item We explicitly incorporate blocks as groups into the pruning formulation to allow the model to prune at both channel and block levels, enabling large pruning ratios.
    \item We introduce layer latency matrices that captures latency variations of each layer to precisely guide the pruning process to meet the target latency budget.
    \item We organically combine the above strategies with a novel pruning framework redefining pruning as a Mixed-Integer Nonlinear Program (MINLP) which directly solves a globally optimal pruned structure within specific latency constraints.
    \item The framework is capable of pruning the model in just one step,  significantly streamlining the entire pruning process.
    \item We conduct a series of detailed experiments across various datasets and model architectures and consistently observe state-of-the-art accuracy-latency trade-offs, especially at large pruning ratios.
\end{itemize}



==> sec_cached/2_related.tex <==
% A plethora of pruning methods has yielded profound progresses in model compression~\cite{lecun1990optimal, han2015deep, gale2019state, zhou2021effective, sun2022disparse}, providing practical speedup and memory benefits~\cite{li2017pruning, molchanov2019importance, he2020learning, lin2020hrank} through hardware-friendly sparsity~\cite{wu2020constraint, li2020eagleeye, shen2021halp, humble2022soft, shen2023hardware} that trades off accuracy and performance  via FLOPs/latency. Our work can be categorized into the field of model pruning. In this section, we will provide a recap of pruning and discuss the latest methods in the field.
\section{Related Works}
\label{sec:related}
\textbf{Pruning}
  Our work can be categorized as a pruning method. We will now provide a brief overview of the field and highlight our differences from the previous approaches. Based on the sparsity pattern, pruning methods can be categorized into unstructured pruning and structured pruning. \textbf{Unstructured pruning} removes individual neurons or weight connections of less significance without consideration for where they occur within each tensor. Parameter significance is usually evaluated on pretrained dense model with a designed importance criterion like  weight magnitude, Hessian-based scores~\cite{lecun1990optimal, hassibi1992second} and probability-based scores~\cite{zhou2021effective, srinivas2017training, molchanov2017variational}. Pruning is usually followed by an additional finetuning for accuracy recovery. On the other hand, \textbf{structured pruning} methods operate under structural constraints, for example removing convolutional filters\cite{li2017pruning} or attention heads\cite{michel2019sixteen}, thus enjoy immediate performance improvement without specialized hardware or library support. Exemplary channel importance criterion relied on metrics like weight norm~\cite{li2017pruning, chin2020towards, he2020learning, he2018soft, yang2018netadapt}, Taylor expansion~\cite{lin2018accelerating, molchanov2019importance, you2019gate}, geometric median~\cite{he2019filter}, and feature maps rank~\cite{lin2020hrank}. In this paper, we focus on \emph{\textbf{structural sparsity}} and leverage the Taylor~\cite{molchanov2019importance} score to estimate parameter importance. 

  Almost all methods~\cite{han2015deep, lin2020hrank, molchanov2019importance, shen2021halp, humble2022soft, he2019filter} perform pruning in an iterative manner, gradually reducing the model size with a designed scheduler like ~\cite{de2020progressive}. Though requiring extra hyper-parameters and tuning efforts, iterative pruning has been claimed to achieve better performance than one-shot pruning. In this paper, we theoretically and empirically demonstrate that our method can be performed with \emph{\textbf{only one shot}}, greatly simplifying the pruning procedure while attaining state-of-the-art results.
  
  \textbf{Hardware-aware Pruning} Since parameter compression ratio does not directly translate into computation reduction ratio, some works~\cite{li2020eagleeye, wu2020constraint, yang2018netadapt} focus primarily on reducing model FLOPs. Latest methods go one step further and perform hardware-aware pruning which aims to directly reduce the hardware inference latency. The representative work HALP~\cite{shen2021halp} first prepares a latency lookup table for all configurations of prunable parameters measured on the target hardware then formulate pruning as a knapsack problem~\cite{sinha1979multiple}, maximizing total parameter importance while constraining the total associated latency under a given budget. ~\cite{shen2023hardware} later demonstrates that HALP can be applied to autonomous systems to achieve real-time detection performance. To enhance the learning capacity of pruned models, SMCP~\cite{humble2022soft} introduces soft masking within the HALP framework, enabling the reconsideration of earlier pruned weights in an iterative pruning setting. 
  
  Although these methods~\cite{shen2021halp, shen2023hardware, humble2022soft} deliver notable gains in accuracy and speedup across various datasets, they face challenges with significant latency reduction or one-shot pruning. These limitations primarily stem from two factors. Firstly, their optimization frameworks lack accuracy as they do not consider all variables impacting parameter latency. For instance, the inference latency of a convolutional layer can be influenced by two prunable parameters: the number of input channels and output channels, yet these methods only account for the latter in their mathematical modeling. Secondly, they struggle to handle hierarchical changes in pruning, such as removing an entire residual block. Remarkably, this hierarchical unawareness is also a common issue in most pruning works~\cite{molchanov2019importance, he2019filter, lin2020hrank, wimmer2022interspace, li2023differentiable}. In this paper, we also focus on the \emph{\textbf{hardware-aware pruning}} setting and present a novel pruning framework that effectively addresses all the above issues with enhanced optimization formulation.

  \textbf{Mixed-Integer Nonlinear Program (MINLP)~\cite{lee2011mixed, burer2012non, bussieck2003mixed}} Since the backbone of our proposed formulation is a MINLP, we will now briefly introduce the field. Formally defined in ~\cite{lee2011mixed}, MINLPs are optimization problems where some of the variables are constrained to take integer(v.s. float) values and the objective and constraints are described by nonlinear functions. Effectively and efficiently solving MINLP~\cite{bonami2008algorithmic, d2013mixed, gunluk2010perspective, duran1986outer, fletcher1994solving, bonami2009feasibility, bernal2020improving} has been a very important topic in optimization research, and key component is usually decomposing the problem into Mixed-Integer Linear Programs (MILP) and Nonlinear Programs (NLP). The representative approach OA~\cite{duran1986outer,fletcher1994solving} performs this by solving an alternating finite sequence of NLP subproblems and relaxed versions of MILP master program. Recently, conveniently modeling and solving MINLPs in Python has been made possible with Pyomo~\cite{bynum2021pyomo} and MindtPy~\cite{bernal2018mixed}.  In this paper, we solve our pruning MINLP using OA~\cite{duran1986outer,fletcher1994solving} with Pyomo~\cite{bynum2021pyomo} and MindtPy~\cite{bernal2018mixed}
  
  % Though achieving decent accuracy and speedups on various datasets, these methods~\cite{shen2021halp, shen2023hardware, humble2022soft} start to exhibit severe performance drops with large latency reduction ratio or one-shot pruning, which are limited by two main criteria. First, their optimization framework itself is inaccurate and does not include all variables affecting parameter latency. For example, inference latency of a convolution layer can be characterized by two prunable parameters: number of input channels and output channels, whereas they~\cite{shen2021halp, humble2022soft, shen2023hardware} only include the number of output channels into their mathematical modeling. Second, they are incapable of handling hierarchical changes in pruning, like the removal of an entire residual block. Notably, we find that this hierarchical unawareness is also a common issue in almost all other pruning methods~\cite{molchanov2019importance, he2019filter, lin2020hrank, wimmer2022interspace, li2023differentiable}. Our work also focuses on the hardware-aware pruning setting and presents a novel pruning framework that effectively addresses the above issues.


==> sec_cached/3_method.tex <==
\section{Methodology}
We will now present our pruning framework. We begin by establishing the relevant notations, followed by a discussion on parameter importance estimation and the creation of the latency lookup table.  Subsequently, we briefly discuss the issues in previous methods~\cite{shen2021halp, shen2023hardware, humble2022soft}. We conclude with the presentation of our enhanced MINLP-based optimization formulation.
\subsection{Preliminaries}
\textbf{Notations} 
For the neural network with $L$ layers in total, we represent its parameters as $\Theta = \bigcup_{l=1}^{L} \Theta_{l},\Hquad \textrm{s.t.}  \Theta_{l} \in \mathbb{R}^{m_{l} \times n_{l} \times K_{l} \times K_{l}}$, where $m_l, n_l, K_l$ represent the number of output channels, input channels, and kernel size at layer $l$ respectively. We define $p_l, p_l \leq m_l$ as the active number of channels at layer $l$ , for example the kept after pruning. Following ~\cite{he2016deep, luo2020neural}, a block is defined as the set of layers(e.g. bottleneck~\cite{he2016deep}) skipped by a residual connection. Suppose there is a total of $B$ blocks in the model. We use $\beta(l), 1\leq \beta(l) \leq B$ to denote the block id that layer $l$ belongs to. Inversely, we also have $\beta^{-1}(b)$ mapping a block ID $b$ to layers contained in it. Moreover, suppose the maximum inference latency we allow for the pruned model is $\Psi$ on a target hardware. 

% \Hquad\sum_{j=1}^{m_l} y_l^j = p_l$

\textbf{Channel Importance Estimation} To represent how important channel $\Theta^j_l$ is to the overall model performance, following ~\cite{shen2021halp, humble2022soft, shen2023hardware}, we leverage the Taylor score~\cite{molchanov2019importance}:
\begin{align}
\label{eqn:importance}
    \mathcal{I}_l^j = |g_{\gamma_l^j}\gamma_l^j + g_{\beta_l^j}\beta_l^j|,
\end{align}
where $\gamma$ and $\beta$ are BatchNorm layer's weight and bias for the corresponding channel, and $g_\gamma$ and $g_\beta$ are the gradients.

\textbf{Latency Lookup Table} 
\label{method-lut}
To reflect the latency reduction of pruning a channel at certain layers, a latency lookup table $\mathcal{T}$ is pre-built same as ~\cite{shen2021halp, shen2023hardware, humble2022soft}. Specifically, $\mathcal{T}_l(p_{l-1}, p_l)$ records the latency at layer $l$ with $p_{l-1}$ active input channels and $p_l$ active output channels.

\textbf{Prior Methods and Weakness} 
\label{method-prior}
Prior methods~\cite{shen2021halp, shen2023hardware, humble2022soft} compute a latency cost for the $j$-th channel at the $l$-th layer $\Theta_l^j$ as:
\begin{align}
\label{eqn: latency}
    R_l^j = T_l(p_{l-1}, j) - T_l(p_{l-1}, j-1)
\end{align}
As each channel is associated with a value~\ref{eqn:importance} and a cost~\ref{eqn: latency}, a knapsack problem can be set up to choose channels that maximize the total parameter importance while using the total latency smaller than the budget $\Psi$. As mentioned, this formulation has its weaknesses. First, the cost modeling~\ref{eqn: latency} is inaccurate since it only accounts for the output channels with $j$ being the variable, and $p_{l-1}$ is considered as constant value. Since pruning is performed globally at each layer, active number of channels at layer $l-1$, i.e. $p_{l-1}$, could be changing as well. This reduction in input channels should also be modeled into our optimization. Second, potential hierarchical changes in pruning is not considered. If all channels within a layer are pruned, training will be problematic with a 'disconnected' neural net. 

\subsection{Ours}
\label{subsec:ours}
With the above knowledge, we now present our method, which simultaneously addresses all above issues.

\textbf{Layer Configuration Selection} 
To formulate the configuration of each layer, we introduce binary decision variables $\bigcup_{l=1}^L\bigcup_{j=0}^{m_l} y_l^j, y_l^j\in \{0,1\}$, and $y_l^j$ being $1$ means that we select $j$ output channels for layer $l$. We can further construct a layer configuration vector $\Vec{y_l}$ as:
\begin{align}
\label{eqn:layer_var}
    \Vec{y_l} = [y_l^0, y_l^1, ..., y_l^{m_l}]
\end{align}
Obviously, we could only have one possible configuration for each layer, thus $\Vec{y_l}$ is constrained to be \textbf{\emph{one-hot}} :
\begin{align}
    \Vec{y_l} \cdot \mathbf{1} = 1, \forall l \in [1, L]
\end{align}
In short, $\Vec{y_l}$ encodes number of output channels at layer $l.$
% To indicate a channel being pruned or kept, we introduce binary channel decision variables $\bigcup_{l=1}^L\bigcup_{j=1}^{m_l} y_l^j$, and $y_l^j$ being $0$ means the $j$-th output channel at the $l$-th layer $\Theta_l^j$ is pruned. Similarly, we also introduce block decision variables $\bigcup_{b=1}^\mathcal{B} z_b$, and $z_b$ being $0$ means the entire block $b$ with all its layers $\beta^{-1}(b)$ is removed.

\textbf{Layer Configuration Latency}  To formulate the inference latency at layer $l$ which can be characterized by its number of input $\Vec{y_{l-1}}$ and output channels $\Vec{y_{l}}$, we construct a latency cost matrix $\mathbf{C_l}$ as follows:
\begin{align}
\label{eqn:latv2}
{
  \mathbf{C_l} =
  \left[ {\begin{array}{cccc}
    T(0, 0) & T(0, 1) & \cdots & T(0, m_l)\\
    T(1, 0) & T(1,1) & \cdots & T(1,m_l)\\
    \vdots & \vdots & \ddots & \vdots\\
    T(m_{l-1}, 0) & T(m_{l-1}, 1) & \cdots & T(m_{l-1}, m_l)\\
  \end{array} } \right]
}
\end{align}
The latency cost of layer $l$ can then be determined as:
\begin{align}
    \Vec{y_{l}} \cdot (\Vec{y_{l-1}} \cdot \mathbf{C_l}) ^ T
\end{align}
Compared with prior methods~\cite{shen2021halp, shen2023hardware, humble2022soft} which only consider the contribution of output channels to the layer latency, we also model the variation of input channels into the expression.

\textbf{Layer Configuration Importance} For a particular layer configuration $y^j_l$, which means we keep $j$ output channels for layer $l$, we represent its importance $\hat{\mathcal{I}^j_l}$ by \textbf{\emph{accumulating the $j$ largest}} channel importance scores~\ref{eqn:importance} at layer $l$. Intuitively, for example, if we only want to keep $1$ channel for a layer, we want this channel to be the most critical. This can be formulated as:
\begin{align}
    \mathcal{I}_l^1 &\geq \mathcal{I}_l^2 \geq ... \geq \mathcal{I}_l^{m_l}\\
    \hat{\mathcal{I}^j_l} &= \sum_{i=1}^j \mathcal{I}_l^i, \Hquad\hat{\mathcal{I}^0_l} = 0,
\end{align}
where $\hat{\mathcal{I}^0_l}$ represents importance of selecting $0$ channels for layer $l$ thus is equal to $0$ . We further construct a layer importance vector $\Vec{V_l}$ as follows:
\begin{align}
\label{eqn:impvec}
    \Vec{V_l} = [\hat{\mathcal{I}^0_l}, \hat{\mathcal{I}^1_l}, ..., \hat{\mathcal{I}^{m_l}_l}]
\end{align}
The importance value of layer $l$ can then be determined as:
\begin{align}
    \Vec{y_l}\cdot\Vec{V_l}
\end{align}

\textbf{Hierarchical Pruning and Block Selection} Previous methods~\cite{shen2021halp, humble2022soft, shen2023hardware} did not consider the specific case when all parameters within a layer are pruned away when we target for large latency reduction. Since the neural net gets 'disconnected', training will become problematic with the emergence of NaN losses. In our method, we explicitly prevent this complete pruning of a layer from happening by setting $y_l^0 = 0, \forall l$. However, since layers preceding and following a block are connected by a residual connection, removing all layers of a block at once is safe, and we argue that this potential hierarchical change should be modeled in the pruning optimization problem. To formulate the selection of each block, we introduce binary decision variables $\bigcup_{b=1}^B z_b, z_b\in \{0,1\}$, and $z_b$ being $0$ means that the entire block $b$ with all its containing layers $\beta^{-1}(b)$ are removed.

\textbf{Unified Formulation} Incorporating all the aforementioned components, the hardware-aware pruning problem can be elegantly represented with a Mixed-Integer Nonlinear Programming (MINLP) formulation:
\begin{align}   
\label{eqn:program}
\argmax_{\bigcup_{l=1}^L \bigcup_{j=0}^{m_l} \{y_l^j\}, \bigcup_{b=1}^B \{z_b\}} & \quad \sum_{l=1}^L  z_{\beta(l)} \times (\Vec{y_l}\cdot\Vec{V_l}) \\
\textsc{s.t.}\quad \sum_{l=1}^L  z_{\beta(l)} \times & (\Vec{y_{l}} \cdot (\Vec{y_{l-1}} \cdot \mathbf{C_l}) ^ T) \leq \Psi \nonumber \\
y_l^j \in \{0, 1\} &,\Hquad\forall l\in [1, L], \forall j\in [0, m_l] \nonumber \\
 z_b \in \{0, 1\} &, \Hquad\forall b\in [1, B] \nonumber \\
    y_l^0 = 0, \Hquad \Vec{y_l} &\cdot \mathbf{1} = 1, \Hquad\forall l\in [1, L] \nonumber 
    % & \Vec{y_l} \cdot \mathbf{1} = 1,\Hquad \forall l \in [1, L]
\end{align}

% \texttt{No Layer Prune Constraint}
% & \Vec{y_s} = \Vec{y_t}, \forall s, t \in \gamma^{-1}(g), \forall g \in [1, G], \texttt{Group Constraint}
The objective here is to jointly determine the best layer and block configurations($y_l^j$ and $z_b$) that maximize the cumulative importance score while ensuring the inference latency remains below the budget $\Psi$. Concretely, this is a cubic program, as the latency constraint is defined through the product of three decision variables. The problem is mixed-integer in nature because we restrict all decision variables to binary values, while the importance vector $\Vec{V}_l$ and latency matrix $\mathbf{C_l}$ contain floating-point numbers. We can also observe from the formulation~\ref{eqn:program} that the block decision variables $z_b$s are given higher 'priority' than the layer decision variables $y_l^j$s.  This is because deactivating $z_b$ results in the exclusion of all layers within block $b$ by zeroing their importance and latency expression, regardless of the values of their layer decision variables $y_l^j$s. Since we are jointly optimizing all the variables, we can directly determine a globally optimal pruned structure with only a single shot,  significantly improving the prior methods~\cite{shen2021halp, shen2023hardware, humble2022soft}. 

In order to solve  this MINLP~\ref{eqn:program}, we leverage the Python-based numerical decomposition framework Pyomo~\cite{bynum2021pyomo} and MindtPy~\cite{bernal2018mixed}. Additionally, we employ the Feasibility Pump (FP) method~\cite{bonami2009feasibility} to enhance the solving process. For instance, when applied to a model like ResNet50~\cite{he2016deep}, the entire optimization problem can be efficiently solved in approximately five seconds on a \AS{check CPU type on NGC}. 

In practice, since the Taylor score~\cite{molchanov2019importance} is measured using gradient information computed from data batches, we perform this single step of pruning at the end of the first finetuning epoch after the model has seen all of the samples in the dataset and accumulate their importance estimation. We then prune according to the configuration variables $y_l^j$ and $z_b$ determined by the solver and finetune the pruned model to recover accuracy. An algorithmic description of the above process is provided in Algorithm~\ref{algo:pseudocode}.
\begin{algorithm}[t]
    \caption{Ours Pseudocode}\label{euclid}
    \label{algo:1}
    \textbf{Input:} Pretrained weights $\Theta$, latency lookup table $T$, total finetuning epochs $E$, training dataset $\mathcal{D}$, latency budget $\Psi$
    \begin{algorithmic}[1]
        \State{\texttt{//Prepare Importance Score}}
        \For{sample $(x, y)$ in $\mathcal{D}$}
        \State{Perform forward pass and backward pass with $\Theta$}
        % \For{$l \in [1, L]$ and $j\in[1, m_l]$}
        \State{Calculate and accumulate importance $\mathcal{I}_l^j$ (Eqn.~\ref{eqn:importance})}
        \EndFor
        \State{\texttt{//Start Pruning}}
        \State{Construct layer importance vector $\Vec{V}_l$ (Eqn.\ref{eqn:impvec})}
        \State{Construct layer latency cost matrix $\mathbf{C}_l$ (Eqn.\ref{eqn:latv2})}
        \State{Declare layer selection variable $\Vec{y}_l$ (Eqn.\ref{eqn:layer_var})}
        \State{Declare block selection variable $z_b$}
        \State{Solve the MINLP (Eqn. \ref{eqn:program}) with Pyomo and MindtPy}
        \State{Prune according to the solver output $\Vec{y}_l$ and $z_b$}
        \State{\texttt{//Finetuning}}
        \State{Finetune the pruned model as usual for $E$ epochs}
    \end{algorithmic}
    \label{algo:pseudocode}
\end{algorithm}

% Although we prevent layers from getting completely pruned, the block decision variables with higher priority will remove the entire 

==> sec_cached/4_exp.tex <==
\section{Experiments}

To validate our proposed method, we perform extensive experiments across a comprehensive set of scenarios. We demonstrate our pruning results on the image classification task with ImageNet~\cite{deng2009imagenet} and ResNet50~\cite{he2016deep}, on the 2D object detection task with Pascal VOC~\cite{everingham2010pascal}, and finally on the 3D object detection task with Nuscenes~\cite{caesar2020nuscenes} and StreamPETR~\cite{wang2023exploring}. We observe new state-of-the-art results with our approach obtaining a much better accuracy-latency pareto than prior arts~\cite{shen2021halp, humble2022soft} and many other competitive baselines~\cite{li2020eagleeye, wang2021neural}. To provide a comprehensive analysis, we also conducted an in-depth ablation study, highlighting the contributions of each component in our formulation enhancement.

Additionally, for ResNet50 and SSD, we aimed to optimize their inference latency on the Nvidia TITAN V GPU, which means that the lookup table $T$~\ref{method-lut} is constructed and measured on TITAN V. Notably, when pruning StreamPETR~\cite{wang2023exploring}, we adapted our approach to target the Nvidia GeForce RTX 3090 GPU, aligning with the focus of StreamPETR's original paper. This allowed us to fairly evaluate the speedup benefits and demonstrate the generalizability of our method across different hardware platforms.

All of our experiments are run on 8 Nvidia Tesla V100 GPUs and conducted with PyTorch~\cite{paszke2017automatic} V1.4.0. For the pretrained model weights to apply our pruning method, we utilized official release checkpoints provided by the authors or those available from the PyTorch model zoo for consistency and reliability.

\textbf{Results on ImageNet}
In Table~\ref{table:imageresnet50}, We report our pruning results and comparison with the baseline methods on ResNet50~\cite{he2016deep} and ImageNet~\cite{deng2009imagenet}. We evaluate these results using Top-1 Accuracy and Top-5 Accuracy to gauge the recovered accuracy after fine-tuning. In addition, we include inference FPS (im/s, i.e. images per second) to directly showcase the speedups on the target hardware. We also present FLOPs for completeness.

Compared with previous methods like HALP~\cite{shen2021halp} and SMCP~\cite{humble2022soft}, we achieve a significantly improved accuracy-latency trade-off. For instance, SMCP reaches a Top-1 accuracy of $72.7$ with an inference speed of $3784$ im/s; our method slightly surpasses its Top-1 with an accuracy of $\mathbf{72.8}$ but with a considerably faster inference speed of \textbf{4210} im/s. While HALP achieves a Top-1 accuracy of $68.6$ with an inference speed of $4101$ im/s, our method significantly outperforms it with a Top-1 accuracy of $\mathbf{70.0}$ and an impressive FPS of $\mathbf{5262}$ im/s. Notably, we can observe from Table~\ref{table:imageresnet50} that our method particularly excels when targeting high FPS with substantial pruning from pre-trained models, corroborating the advantages of our enhanced optimization formulation as discussed in~\ref{subsec:ours}.
 
\begin{table*}[ht!]
    \centering
    \vspace{-0.2cm}
    % \resizebox{.85\textwidth}{!}
    {
        % \begin{tabular}{c|cccc}
        \begin{tabular}{lcccc}
            \toprule
            \rowcolor{lgray} 
            \textsc{Method} & \textsc{Top-1 Acc}($\%$)$\uparrow$ & \textsc{Top-5 Acc}($\%$)$\uparrow$  & \textsc{FLOPs}($\times e^9$)$\downarrow$ & \textsc{FPS(im/s)}$\uparrow$ \\
            % {\footnotesize (baseline)}
            \midrule
            \multicolumn{5}{c}{\textbf{ResNet50~\cite{he2016deep}}}\\
            \textsc{Dense} & $76.2$&$92.9$ & $4.1$&$1019$\\
            \midrule
            \textsc{MetaPrune}\cite{liu2019metapruning} & $73.4$ & --& $1.0$ & $2381$ \\
            \textsc{AutoSlim}\cite{yu2019autoslim} & $74.0$ & --& $1.0$ & $2390$ \\
            \textsc{GReg-2}\cite{wang2021neural} & $73.9$ & --& $1.3$ & $1514$ \\
            \textsc{HALP-$30\%$}\cite{shen2021halp} & $74.5$ &$91.8$ & $1.2$ & $2597$ \\
            \textsc{SMCP-$30\%$}\cite{humble2022soft} & $\mathbf{74.6}$ &$92.0$ & $1.0$ & $2947$ \\
            %\textsc{HALP*-$30\%$} & $74.5$ &$92.0$& $1.1$ & $2488$ & $90+90$&\cmark\\
            \rowcolor{lgreen} \textbf{\textsc{Ours-30\%}} & $\mathbf{74.6}$ &$\mathbf{92.2}$ & $1.1$ & $\mathbf{3092}$ \\
            \midrule
            \textsc{HALP-$15\%$}\cite{shen2021halp} & $68.1$ &$88.4$& $0.6$ & $3971$ \\
            \rowcolor{lgreen} \textbf{\textsc{Ours-15\%}} & $\mathbf{70.0}$ &$\mathbf{89.3}$& $0.5$ & $\mathbf{5306}$ \\
            \midrule
            \midrule
            \multicolumn{5}{c}{\textbf{ResNet50 - EagleEye~\cite{li2020eagleeye}}}\\
            \textsc{Dense}~\cite{li2020eagleeye} & $77.2$ &$93.7$& $4.1$&$1019$\\
            \bottomrule
 \textsc{EagleEye-1G}\cite{li2020eagleeye} & $74.2$ &$91.8$ & $1.0$ & $2429$ \\
 \textsc{HALP-30\%}\cite{shen2021halp} & $74.5$ &$91.9$ & $1.2$ & $2597$ \\
  \textsc{SMCP-30\%}\cite{humble2022soft} & $75.1$ &$92.3$ & $1.1$ & $2589$ \\
    \rowcolor{lgreen}
  \textbf{\textsc{Ours-35\%}} & $\mathbf{75.2}$ &$\mathbf{92.5}$& $1.3$ & $\mathbf{2774}$ \\
  \rowcolor{lgreen}
  \textbf{\textsc{Ours-30\%}} & $75.0$ &$92.2$& $1.2$ & $3052$ \\
  \midrule
  % \textsc{SMCP-25\%}\cite{humble2022soft} & $74.4$ &$92.0$ & $0.9$ & $3102$ \\
  \textsc{HALP-20\%}\cite{shen2021halp} & $71.2$ &$90.1$& $0.7$ & $3691$ \\
  \textsc{SMCP-20\%}\cite{humble2022soft} & $72.7$ &--& --& $3784$ \\
  \rowcolor{lgreen}
  \textbf{\textsc{Ours-20\%}} & $\mathbf{72.8}$ &$\mathbf{90.9}$& $0.7$ & $\mathbf{4210}$ \\
  \midrule
\textsc{HALP-15\%}\cite{shen2021halp} & $68.6$ &$88.5$& $0.6$ & $4101$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-15\%}} & $\mathbf{70.0}$ &$\mathbf{89.2}$& $0.5$ & $\mathbf{5262}$ \\
\bottomrule
        \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\textbf{ImageNet results with ResNet-50}. FPS is measured on NVIDIA TITAN V. Results with similar FPS are grouped. Ours achieve much better accuracy-FPS tradeoffs than the baselines, specifically when pruning ratio is large. Averaged results over two runs. \AS{Forgot to get TOP-5 from my training logs. Need to connect with someone to get those data.}}
    \vspace{-0.2cm}
    \label{table:imageresnet50}
\end{table*}

\begin{figure}[ht!]
\begin{center}
   \includegraphics[width=\linewidth]{figs/pascalvoc.pdf}
\end{center}
\vspace{-5pt}
\caption{\textbf{PascalVOC results with SSD512}. Results of FPS versus mAP are plotted (left, top-right is better). FPS is measured on NVIDIA TITAN V. Ours achieve much better accuracy-FPS tradeoffs than the baselines.}
\label{fig:pascal}
\end{figure}
\textbf{Results on PascalVOC} 
% To demonstrate the generalizability of our approach, we also conduct experiments on 2D detection with the popular Pascal VOC~\cite{everingham2010pascal} dataset. 
% In Figure~\ref{fig:pascal}, We report our results of pruning a SSD512~\cite{liu2016ssd} with a ResNet50 backbone and compare with several competitive baselines including HALP~\cite{shen2021halp} and SMCP~\cite{humble2022soft}. We showcase the Pareto frontier of FPS versus mAP. Ours clearly outperforms other methods in the literature by a significant margin. Compared with SMCP, we are able to achieve much higher mAP at similar inference FPS. Notably, our pruned model even surpasses the mAP of pre-trained dense SSD512-RN50 while significantly improving its FPS.
To illustrate the broad applicability of our approach, we also conducted experiments in the realm of 2D object detection using the widely recognized Pascal VOC dataset~\cite{everingham2010pascal}. In Figure~\ref{fig:pascal}, we present the outcomes of our pruning methodology applied to an SSD512~\cite{liu2016ssd} model with a ResNet50 backbone. Our performance is assessed against various competitive baselines, including HALP~\cite{shen2021halp} and SMCP~\cite{humble2022soft}. We depict the Pareto frontier, showcasing the trade-off between FPS and mean Average Precision (mAP).

Our results distinctly outshine existing methods in the field, marking a substantial advancement. In direct comparison to SMCP, our approach consistently achieves significantly higher mAP scores across various inference FPS levels. For instance, we outperform SMCP with an mAP of $\mathbf{79.2}$ (compared to $78.3$) while also slightly increasing the FPS to $\mathbf{146.4}$ (compared to $144.4$).Notably, our pruned model even surpasses the mAP of the pre-trained dense SSD512-RN50 by a margin($\mathbf{80.0}$ v.s. $78.0$)while substantially enhancing its FPS($\mathbf{125.4}$ v.s. $68.2$).
% We further demonstrate the generalizability of our approach to object detection task. Settings and hyperparameters are detailed in the supplemental material. We report our results of pruning a SSD512~\cite{liu2016ssd} using a ResNet50 backbone on the popular PASCAL VOC dataset~\cite{everingham2010pascal} in Figure. \ref{fig:detection_cmp}. As shown, LookAhead clearly outperforms other methods in the literature with higher accuracy and/or a faster FPS, and even surpasses the dense model with doubled inference speed.

% *Benefited from the perspective-view pre-training. †300 randomly initialized queries and 128 propagation queries. † Offline method using future frames.
\begin{table*}[ht!]
\centering
\begin{tabular}{c|c|c|ccccc|c}
\toprule
\rowcolor{lgray}
\textsc{Method} & \textsc{mAP$\uparrow$} & \textsc{NDS$\uparrow$} & \textsc{mATE$\downarrow$} & \textsc{mASE$\downarrow$} & \textsc{mAOE$\downarrow$} & \textsc{mAVE$\downarrow$} & \textsc{mAAE$\downarrow$} & \textsc{FPS$\uparrow$} \\
\midrule
\textsc{BEVPoolv2}\cite{huang2022bevpoolv2} & $0.406$ & $0.526$ & $0.572$ & $0.275$ & $0.463$ & $0.275$ & $0.188$ & $16.6$ \\
\textsc{BEVDet4D}\cite{huang2022bevdet4d}& $0.322$ & $0.457$ & $0.703$ & $0.278$ & $0.495$ & $0.354$ & $0.206$ & $16.7$ \\
\textsc{PETRv2}\cite{liu2023petrv2} & $0.349$ & $0.456$ & $0.700$ & $0.275$ & $0.580$ & $0.437$ & $0.187$ & $18.9$ \\
\textsc{Sparse4Dv2}\cite{lin2023sparse4d} & $0.439$ & $0.539$ & $0.598$ & $0.270$ & $0.475$ & $0.282$ & $0.179$ & $20.3$ \\
\textsc{StreamPETR}\cite{wang2023exploring} & $0.449$ & $0.546$ & $0.613$ & $0.267$ & $0.413$ & $0.265$ & $0.196$ & $31.7$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-55\%}} & $\mathbf{0.451}$ & $\mathbf{0.551}$ & 0.596& 0.272& 0.413& $0.259$& $0.207$& $\mathbf{37.3}$ \\
\midrule
\textsc{HALP-50\%}~\cite{shen2021halp} & $0.439$ & $0.543$ & 0.605 & 0.270 & 0.419 & 0.265 & 0.211 & $38.6$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-50\%}} & $\mathbf{0.441}$ & $\mathbf{0.544}$ & 0.606 & 0.269 & 0.421 & 0.268 & 0.205& $\mathbf{39.0}$ \\
\midrule
\textsc{HALP-40\%}~\cite{shen2021halp} & $\mathbf{0.427}$ & $\mathbf{0.533}$ & 0.620 & 0.269 & 0.438 & 0.271 &0.209 &$39.5$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-40\%}} & $\mathbf{0.427}$ & $0.532$ & 0.608 &  0.272 & 0.457 &0.269 &0.207 & $\mathbf{40.7}$ \\
\midrule
\textsc{HALP-30\%}~\cite{shen2021halp} & $0.373$ & $0.489$ & 0.674 & 0.277 & 0.534 & 0.293 & 0.197 & $42.5$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-30\%}} & $\mathbf{0.394}$ & $\mathbf{0.512}$ & 0.642 & 0.275 & 0.449 & 0.278 & 0.204 & $\mathbf{43.3}$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Nuscenes results with StreamPETR}. FPS is measured on NVIDIA GeForce RTX 3090. Results with similar FPS are grouped. Ours achieve much better accuracy-FPS tradeoffs than HALP and even surpass performance of dense StreamPETR with much higher FPS. \AS{Forgot to get those mean error stats from my training logs. Need to connect with someone to get those data.}}
\label{table:nuscenes}
\end{table*}
\textbf{Results on Nuscenes}
We further conducted a comprehensive evaluation of our methodology in the challenging task of 3D object detection, utilizing the widely recognized Nuscenes dataset~\cite{caesar2020nuscenes} and the latest State-of-the-art model StreamPETR~\cite{wang2023exploring}. Notably, our work marks the first instance of pruning tailored specifically for this application in the field. Detailed results and comparisons with several competitive baselines are presented in Table ~\ref{table:nuscenes}. Our evaluation incorporated a diverse set of evaluation metrics commonly adopted for 3D object detection tasks~\cite{caesar2020nuscenes, wang2023exploring, lin2023sparse4d}, including the mean Average Precision (mAP) and Normalized Detection Score (NDS). Additionally, we report the FPS to highlight the improvements in speed.

Significantly, when compared to the dense pre-trained StreamPETR model, our technique achieved a substantial acceleration of approximately $18\%$, resulting in an impressive $\mathbf{37.3}$ FPS as opposed to the baseline's $31.7$ FPS. Importantly, this speed boost was achieved without sacrificing performance: our pruned model attained superior mAP ($\mathbf{0.451}$ vs. $0.449$) and NDS ($\mathbf{0.551}$ vs. $0.546$). In comparison to the previous pruning method HALP~\cite{shen2021halp}, our approach exhibited remarkable improvements in accuracy-latency trade-offs across various pruning ratios. For instance, HALP managed to produce a pruned StreamPETR model with an mAP of $0.373$, an NDS of $0.489$, and an inference FPS of $42.5$. In contrast, our approach surpassed these results, achieving an mAP of $\mathbf{0.394}$, an NDS of $\mathbf{0.512}$, and an inference FPS of $\mathbf{43.3}$.

\subsection{Ablation Study and More}
\textbf{One-shot versus Iterative Pruning} Previous methods like HALP~\cite{shen2021halp} start to exhibit severe performance drops when we aim for larger latency reduction from the model or pruning in one shot due to the issues we discussed in Sec.~\ref{method-prior}. In Table~\ref{table:imageresnet50}, we can concretely see from the results that HALP indeed fails to achieve competitive performance at large latency reduction. Here, in Table~\ref{table:ablation}, we demonstrate the variations of performance of HALP and ours over different pruning steps. To clarify, "pruning steps" refer to the number of steps taken to achieve the desired pruned latency. A one-shot pruning approach, like ours, directly meets the target latency, resulting in a pruning step count of $1$. In contrast, HALP employs an exponential prune scheduler~\cite{de2020progressive}, reaching the target latency over $30$ pruning steps, which requires extra computation and hyperparameter tuning efforts. As observed in Table~\ref{table:ablation}, HALP's performance deteriorates as the pruning step count reduces. In the most extreme scenarios of one-shot pruning, HALP fails dramatically, over-pruning significantly and not adhering to the desired pruning ratio and latency budget. Such issues arise because HALP's suboptimal formulation , as mentioned in ~\ref{method-prior}, overlook the consequences of input channel reductions in latency. While these weaknesses can be somewhat mitigated with a large number of pruning steps, they become more pronounced with only one or a few steps. In stark contrast, our approach maintains robust performance, irrespective of whether it's one-shot or iterative pruning.

\textbf{Ablation of Each Component} 
As presented in ~\ref{subsec:ours}, our method has two major differences from previous methods~\cite{shen2021halp, shen2023hardware, humble2022soft} which allow us to outperform especially in contexts of significant latency reduction and single-shot pruning. Firstly, we set up a \textbf{nonlinear pruning formulation} which jointly optimizes all the variables impacting model latency and importance. This allows us to identify an optimal pruned structure in a single pruning step. Second, we explicitly formulate the selection of each ``block". This aids in managing the \textbf{hierarchical change} during pruning, resulting in a more refined structure. 

To delve deeper into our method, we've examined two variants where each component operates independently to understand their respective impacts on pruning performance. Detailed formulations of these two variants are included in our supplementary material. We conduct these ablation experiments on ImageNet with ResNet50 and depict the Pareto frontier of FPS versus Top-1 in Figure~\ref{fig:ablation}. Additionally, we include the performance of HALP~\cite{shen2021halp} and ours for a clearer perspective. In the \textbf{\emph{Ours-Only Nonlinear Global}} (represented in purple in Figure~\ref{fig:ablation}), we retain the nonlinear formulation but exclude the block formulation. Conversely, in the \textbf{\emph{Ours-Only Hierarchical}} (shown in cyan in Figure~\ref{fig:ablation}), we adopt HALP's~\cite{shen2021halp} linear latency formulation, but integrate block selection into our optimization. From Figure~\ref{fig:ablation}, it's evident that each of these two changes results in a markedly better accuracy-latency tradeoff than HALP. While both modifications have their individual merits, combining them proves even more beneficial. Consequently, our combined approach, illustrated in green in Figure~\ref{fig:ablation}, unsurprisingly delivers the most optimal performance when we integrate both enhancements, with a unified formulation~\ref{eqn:program}.
% Although our method is one-shot, we also present 



\begin{table}[t!]
\centering
\begin{tabular}{c|clcc}
\toprule
\rowcolor{lgray}
\textsc{Method} & \textsc{Steps} &\textsc{Ratio}& \textsc{Top-1$\uparrow$}& \textsc{FPS$\uparrow$} \\
\midrule
\textsc{HALP}\cite{shen2021halp} & $30$  &70& $74.3$ & $2505$ \\
\textsc{HALP}\cite{shen2021halp} & $10$  &70& $73.9$ & $2622$ \\
\textsc{HALP}\cite{shen2021halp} & $1$  &70& $65.1$ & $4444$ \\
\hdashline
\textbf{\textsc{Ours}} & $30$  &70& $74.5$ & $2660$ \\
\textbf{\textsc{Ours}} & $10$  &70& $74.8$ & $2860$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours}} & $1$  &70& $75.2$ & $2774$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation study results on ImageNet with ResNet50}. Results of HALP~\cite{shen2021halp} and ours with different pruning steps are shown with a pruning ratio of $70\%$. One-shot pruning correspond to Steps of 1. HALP is completely not functioning with one-shot or smaller pruning steps.}
\label{table:ablation}
\end{table}

\begin{figure}[t!]
\begin{center}
   \includegraphics[width=\linewidth]{figs/Ablation3.pdf}
\end{center}
\vspace{-5pt}
\caption{\textbf{Abaltion study results on ImageNet with ResNet50}. We ablate on our method and show the results of each component of our formulation operating independently. Top-right is better.}
\label{fig:ablation}
\end{figure}

\begin{figure}[t!]
\begin{center}
   \includegraphics[width=\linewidth]{figs/Softmasking.pdf}
\end{center}
\vspace{-5pt}
\caption{\textbf{Results of ours with soft masking on ImageNet with ResNet50}. We investigate the effectiveness of soft masking techniques in our method and observe improvement in Top1 at a high FPS level. Top-right is better.}
\label{fig:softmaskg}
\end{figure}

\textbf{Soft Masking}
Recent advances in pruning~\cite{humble2022soft, zhou2021learning, he2018soft, kusupati2020soft, kim2021dynamic} have increasingly adopted soft masking techniques to retain the learning capacity of pruned models by not directly removing the pruned weights. Notably, SMCP~\cite{humble2022soft} integrates this method into the HALP hardware-aware pruning framework, resulting in an enhanced accuracy-latency tradeoff for pruned models. Here, we explore the potential of soft masking to enhance our model's performance. Comprehensive details on the integration and formulation of this approach can be found in our supplementary materials.

We conduct this study on ImageNet with ResNet50 and depict the Pareto frontier of FPS versus Top-1 in Figure~\ref{fig:softmaskg}. For clarity, we also include the performance of SMCP~\cite{humble2022soft} and ours. The results reveal that soft masking offers limited advantages at lower FPS levels with modest pruning ratios and latency reduction. Nonetheless, targeting higher FPS levels leads to notable improvements in Top-1 accuracy. This outcome may be attributed to the Taylor channel importance score we employed~\cite{molchanov2019importance}, which gauges parameter significance based on its impact on loss. Though it maintains precision with minor parameter deletions, its reliability may diminish when a larger number of parameters are pruned concurrently. The iterative reassessment inherent to the soft masking technique may counteract this shortcoming.

% \begin{table*}[ht!]
%     \centering
%     \vspace{-0.2cm}
%     \resizebox{.85\textwidth}{!}
%     {
%         % \begin{tabular}{c|cccc}
%         \begin{tabular}{lcccc}
%             \toprule
%             \rowcolor{lgray} 
%             \textsc{Method} & \textsc{mAP}$\uparrow$& \textsc{NDS}$\uparrow$& \textsc{mATE}$\downarrow$& \textsc{FPS(im/s)}$\uparrow$ \\
%             % {\footnotesize (baseline)}
%             \midrule
%             \multicolumn{5}{c}{\textbf{ResNet50~\cite{he2016deep}}}\\
%             \textsc{Dense} & $76.2$&$92.9$ & $4.1$&$1019$\\
%             \midrule
%             \textsc{MetaPrune}\cite{liu2019metapruning} & $73.4$ & --& $1.0$ & $2381$ \\
%             \textsc{AutoSlim}\cite{yu2019autoslim} & $74.0$ & --& $1.0$ & $2390$ \\
%             \textsc{GReg-2}\cite{wang2021neural} & $73.9$ & --& $1.3$ & $1514$ \\
%             \textsc{HALP-$30\%$}\cite{shen2021halp} & $74.5$ &$91.8$ & $1.2$ & $2597$ \\
%             \textsc{SMCP-$30\%$}\cite{humble2022soft} & $\mathbf{74.6}$ &$92.0$ & $1.0$ & $2947$ \\
%             %\textsc{HALP*-$30\%$} & $74.5$ &$92.0$& $1.1$ & $2488$ & $90+90$&\cmark\\
%             \rowcolor{lgreen} \textbf{\textsc{Ours-30\%}} & $\mathbf{74.6}$ &$\mathbf{92.2}$ & $1.1$ & $\mathbf{3092}$ \\
%             \midrule
%             \textsc{HALP-$15\%$}\cite{shen2021halp} & $68.1$ &$--$ & $0.6$ & $3971$ \\
%             \rowcolor{lgreen} \textbf{\textsc{Ours-15\%}} & $\mathbf{70.0}$ &$--$ & $0.5$ & $\mathbf{5306}$ \\
%             \midrule
%             \midrule
%             \multicolumn{5}{c}{\textbf{ResNet50 - EagleEye~\cite{li2020eagleeye}}}\\
%             \textsc{Dense}~\cite{li2020eagleeye} & $77.2$ &$93.7$& $4.1$&$1019$\\
%             \bottomrule
%  \textsc{EagleEye-1G}\cite{li2020eagleeye} & $74.2$ &$91.8$ & $1.0$ & $2429$ \\
%  \textsc{HALP-30\%}\cite{shen2021halp} & $74.5$ &$91.9$ & $1.2$ & $2597$ \\
%   \textsc{SMCP-30\%}\cite{humble2022soft} & $75.1$ &$92.3$ & $1.1$ & $2589$ \\
%     \rowcolor{lgreen}
%   \textbf{\textsc{Ours-35\%}} & $\mathbf{75.2}$ &$--$ & $1.3$ & $\mathbf{2774}$ \\
%   % \rowcolor{lgreen}
%   % \textsc{Ours-30\%} & $75.0$ &$--$ & $1.2$ & $3052$ \\
%   \midrule
%   % \textsc{SMCP-25\%}\cite{humble2022soft} & $74.4$ &$92.0$ & $0.9$ & $3102$ \\
%   \textsc{HALP-20\%}\cite{shen2021halp} & $71.2$ &$--$ & $0.7$ & $3691$ \\
%   \textsc{SMCP-20\%}\cite{humble2022soft} & $72.7$ &$--$ & $--$ & $3784$ \\
%   \rowcolor{lgreen}
%   \textbf{\textsc{Ours-20\%}} & $\mathbf{72.8}$ &$--$ & $0.7$ & $\mathbf{4210}$ \\
%   \midrule
% \textsc{HALP-15\%}\cite{shen2021halp} & $68.6$ &$--$ & $0.6$ & $4101$ \\
% \rowcolor{lgreen}
% \textbf{\textsc{Ours-15\%}} & $\mathbf{70.0}$ &$--$ & $0.5$ & $\mathbf{5262}$ \\
% \bottomrule
%         \end{tabular}
%     }
%     \vspace{-0.2cm}
%     \caption{\textbf{ImageNet results with ResNet-50}. FPS is measured on NVIDIA TITAN V. Results with similar FPS are grouped. Ours achieve much better accuracy-FPS tradeoffs than the baselines, specifically when pruning ratio is large. Averaged results over two runs.}
%     \vspace{-0.2cm}
%     \label{table:imageresnet50}
% \end{table*}


==> sec_cached/5_concl.tex <==
\section{Conclusion}

==> sec_cached/intro_cache.tex <==
\section{Introduction}
\label{sec:intro}
In the era of deep learning, the quest for efficient neural network has become increasingly paramount. The challenge lies in obtaining models that not only achieve state-of-the-art performance but are also suitable for deployment on edge devices. These devices face constraints in computational resources, inference latency, memory, and power, which can severely limit their capabilities. In applications like autonomous driving, failure to achieve real-time model inference could pose significant safety concerns.

Model pruning~\cite{han2015deep, li2017pruning, alvarez2016learning,shen2021halp,humble2022soft,molchanov2019importance,lee2018snip, evci2020rigging}, in particular, has garnered significant attention as an effective technique to reduce the computational footprint of deep models without significantly compromising accuracy. It involves removing redundant parameters from a densely pre-trained model and subsequently fine-tuning it. Traditional pruning approaches~\cite{han2015deep, li2017pruning, molchanov2019importance, lin2020hrank, lee2018snip, wang2019picking} are usually focused on maximum parameter removal by designing parameter ``importance scores" aiming to rank the redundant ones the lowest. Some later works~\cite{li2020eagleeye, wu2020constraint,yu2019autoslim} also start to explore and target different computational proxies like Floating Point Operations (FLOPs) to enhance pruning effectiveness. However, recent research, as suggested by ~\cite{tan2019mnasnet, shen2021halp}, has shown that FLOPs are not directly related to hardware latency.  This means that the pruned model may not infer as quickly as expected on the target hardware device.

Recent advancements~\cite{shen2021halp,humble2022soft,castro2022probing,chen2022lap,kong2022spvit,yang2023global,molchanov2022lana,shen2023hardware} in pruning techniques have shifted their focus towards hardware-aware pruning. These methods aim to obtain performant pruned models that directly reduce hardware inference latency, offering practical benefits.  Representative approaches HALP~\cite{shen2021halp} and SMCP~\cite{humble2022soft} start by creating hardware-specific latency lookup tables. They then formulate pruning as a knapsack problem~\cite{sinha1979multiple}, maximizing parameter importance while constraining the associated parameter latency under a preset budget.

While these methods have shown promise in achieving speedup and accuracy, obvious limitations start to emerge when we aim for larger latency reduction from the model or pruning in one shot. These limitations result from their (i) suboptimal optimization problem and (ii) incapability to handle pruning with hierarchical change (e.g. removing a residual block all at once).
% their optimization frameworks have two significant drawbacks. First, they do not consider all variables that affect parameter latency. For instance, the inference latency of a convolution layer can be influenced by two prunable variables: the number of input channels and output channels. They only consider the impacts of reducing the number of output channels. Second, they struggle with hierarchical pruning, such as removing an entire residual block at once from the model. These inaccuracies in optimization formulations result in (i) suboptimal pruning performance, especially for substantial latency reductions, and (ii) an inability to perform one-shot or few-shot pruning.

In this paper, we present a novel and effective pruning framework that re-formulates pruning as a Mixed-Integer Nonlinear Program (MINLP)~\cite{lee2011mixed} to directly solve a \emph{\textbf{globally optimal}} pruned model structure with potential hierarchal change from the original model. Compared with the previous methods, we effectively address (i) and (ii) with optimization formulation enhancement. Furthermore, our framework is able to prune the model with \emph{\textbf{only single shot}}.

In this paper, we aim to simultaneously address (i) and (ii) by re-formulating pruning as a Mixed-Integer Nonlinear Program (MINLP)~\cite{lee2011mixed} to obtain a \emph{\textbf{globally optimal}} pruned model with \emph{\textbf{only single shot}}. We conduct extensive experiments to validate our proposed method and observe state-of-the-art accuracy-latency trade-offs in a wide range of settings, covering (a) ImageNet~\cite{deng2009imagenet} for classification, Pascal VOC~\cite{everingham2010pascal} for 2D detection, and Nuscenes~\cite{caesar2020nuscenes} for 3D detection (b) with three model architectures: ResNet-50~\cite{he2016deep}, SSD~\cite{liu2016ssd}, and StreamPETR~\cite{wang2023exploring} (c) across various latency reduction pruning ratios. Additionally, we conducted a thorough ablation study to showcase the improvement brought by each aspect of our enhanced formulation. We summarize our key contributions as follows:
\AS{to be added}.



% Motivations: 

% The latest state-of-the-art pruning methods focus on hardware-aware acceleration, which tries to obtain a performant sub-network structure from a pre-trained model and directly reduces the hardware inference latency to yield practical benefits. Representative methods are HALP and SMCP, which formulate pruning as a knapsack problem, maximizing parameter importance while constraining the associated inference latency under a pre-set budget. Though they obtained decent results on various datasets, their optimization framework is not optimal and suffers from two major drawbacks. First, the optimization problem itself is globally sub-optimal because it does not include all variables that affect the latency of parameters. For example, the latency of a convolution layer can be characterized by two prunable variables: number of input channels and output channels. Prior methods only consider the impacts brought by reducing the number of output channels. Second, they are incapable of handling hierarchical pruning, which for example directly removes a residual block from the entire architecture. We aim to simultaneously solve both of the two issues by re-formulating pruning as a Mixed-Integer Nonlinear Program which directly solves 
